Orbital stability of two circumbinary planets around misaligned eccentric binaries

With $n$-body simulations we investigate the stability of tilted circumbinary planetary systems consisting of two nonzero mass planets. The planets are initially in circular orbits that are coplanar to each other, as would be expected if they form in a flat but tilted circumbinary gas disc and decouple from the disc within a time difference that is much less than the disc nodal precession period. We constrain the parameters of stable multiple planet circumbinary systems. Both planet-planet and planet-binary interactions can cause complex planet tilt oscillations which can destabilise the orbits of one or both planets. The system is considerably more unstable than the effects of these individual interactions would suggest, due to the interplay between these two interactions. The stability of the system is sensitive to the binary eccentricity, the orbital tilt and the semi-major axes of the two circumbinary planets. With an inner planet semi-major axis of $5\,a_{\rm b}$, where $a_{\rm b}$ is semi-major axis of the binary, the system is generally stable if the outer planet is located at $\gtrsim 8\,a_{\rm b}$, beyond the 2:1 mean motion resonance with the inner planet. For larger inner planet semi-major axis the system is less stable because the von-Zeipel--Kozai--Lidov mechanism plays a significant role, particularly for low binary-eccentricity cases. For the unstable cases, the most likely outcome is that one planet is ejected and the other remains bound on a highly eccentric orbit. Therefore we suggest that this instability is an efficient mechanism for producing free-floating planets.

==> response.tex <==
Dear Scientific Editor and Assistant Editor,

We thank the referee for the useful report that has improved the manuscript.
We have thoroughly reviewed the referee’s comments and made several changes to the manuscript. Referee-prompted changes in the updated document are highlighted in bold text. Additional edits, clarifying our methodology and results, are included, but not highlighted. We hope that you are satisfied with the revised manuscript.

Sincerely,
Cheng Chen, Stephen H. Lubow, Rebecca G. Martin & Chris J. Nixon.

1) Abstract
"The stability of the system is sensitive to the binary eccentricity, the orbital tilt and the semi-major axes of the two circumbinary planets."

While the eccentricities of the planets are assumed as zero in this study, they are also important in terms of orbital stability.

RESPONSE: We thank referee for mentioning the role of the eccentricity of the planet. We added sentences to the abstract and second and third paragraph of Section 2 to make our initial assumptions clear. 


2) Please change the reference of Martin & Fabrycky 2021 from arXiv version to journal version. There are other arXiv references. Please use the journal version for the reference, if possible.

RESPONSE: We thank referee for mentioning it and we have fixed it in References. 


3) "In the current observations, only the Kepler-47 system has multiple CBPs but the binary orbit is nearly circular (e < 0.03) and the three Neptune-size planets are nearly coplanar"
There are other binary systems (TOI-1338, NN Ser, Kepler-451) with multiple CBPs as well.

RESPONSE: Thanks for raising these examples. We have added these three additional circumbinary planetary system at the end of this paragraph.


4) Page 2, line 42, left column:
"Nevertheless, the existence of multiple CPBs around Kepler-34 and Kepler-451 (Esmer et al. 2022) suggests that multi-planet circumbinary systems may be common."
Did the authors mean Kepler-47 instead of Kepler-34? To my knowledge Kepler-34 has 1 planet. 
TOI-1338 can be added to the sentence. Planet b of TOI-1338, detected via transit, and planet c detected via radial velocity. The radial velocity detection is first in a binary system.
However, only two (or three) detections can not suggest that multi-planet circumbinary systems are common.

RESPONSE: Yes, this a typo that we have fixed. We have also added TOI-1338, NN Ser, Kepler-451 in the sentence. To avoid misleading that the multi-circumbinary planetary system are necessarily common, we have rewritten the sentence.  


5) Section 3:
The authors give Eq.4 as a stability criterion for the case of single stars with two planets.
Then in the last paragraph (line 32) they give the stability criterion for the binary case, which depends on the eccentricity and semi-major axis of individual planets. 
Is the criterion of Eq.4 still valid for the case of binary stars? If so, please mention it in a clear way.

RESPONSE: Yes, Eq.4 only valid for two planets around a single star. We have added several sentences to make it clear and explain in section 3. 

6) The following sentence needs to be in the next paragraph, which is about the binary case.

"On the other hand, a single CBP is stable for a p ≳ 5 a b around an equal mass binary system (Chen et al. 2020)."

RESPONSE: We have placed this sentence to the next paragraph.

7) In the text it says that the masses of the binary are equal, but the value of the masses are missing. For example, is m1 = m2 = 1 M_sun? or m1 + m2 = 1 M_sun?

RESPONSE: We have mentioned the mass of the binary at the end of first paragraph in Sec. 2. To make it clearer, we mentioned the total mass of the binary at the beginning in Sec. 3.2. 


8) Section 3.1
Starting from line 46, the authors start to explain Fig. 1, without mentioning the figure.

RESPONSE: We thank the referee for mentioning it. We have mentioned Fig. 1 in the sentence before we start to explain it.



9) Section 3.1
Paragraph starting from line 51.
Is there a specific reason for the authors to run the integrations for 14 million years?


RESPONSE: The reason why we choose the longer integration time = 14×10^6 T_b for a_p1 = 10 a_b simulations and 40 ×10^6 T_b for a_p = 20 a_b simulations is to make sure the inner planet has the same orbital revolution numbers as that with a_p1 = 5 a_b. Thus, we can confirm whether the system is stable or not under the same physical timescale for different cases. We have also added a sentence to address this issue in Sec.3.3.

10) WHFAST is a fixed timestep integrator. But the timesteps that was used in the simulations are missing. Please provide them in the manuscript.

RESPONSE: The timestep we use is 2\% of the orbital period of the inner planet. (We have tested shorter timesteps = 0.2\% and find that 2\% is sufficient to ensure accurate results before we start to run stability map.)  
We added a sentence in the first paragraph of Sec. 2

11) Section 3.1

Assuming two coplanar planets around a single star, and varying their the inclinations with the same amount means that all the system objects are coplanar in all situations.
The objects are point masses and there is no tidal interaction implemented to the simulation. Therefore, it is hard to understand the actual reason for this specific search. What was the authors' expectation with this search?

RESPONSE:  We have added some description of our motivation at the end of the first paragraph in section 3.1. As discussed at the end of Section 3.1, the results are not the same at different inclinations, due to round off errors.


12) For all the stability maps, it would be easier for the reader if the authors plot the resonances as horizontal lines.

RESPONSE: We have added five horizontal lines with different colours in the stability maps and added a sentence to describe them at the second paragraph of Sec. 3.1. and Fig.1.



13) For the binary cases, the authors use scaled semi-major axis values (in a_b units) instead of absolute units (in au). I suggest the authors give an absolute value of a_b (similar to section 3.1) for the sake of reproducibility.

RESPONSE: In the code, we still use the scaled value 1 to represent the absolute value 1 au, as well as the mass of the central star M_{\odot}. We have added sentences to explain it at the first paragraph of Sec. 3.1 

	
14) In Fig 4.
The description of the lower right panel on both sides is mutual inclination of the planets (delta i_p). According to page 6, line 27, left panel, this parameter means the difference of inclination of individual planets (i_p1 - i_p2).

If this parameter is (i_p1 - i_p2), then the range that this parameter oscillates should be around 0 - 10 degrees, according to the middle left panel.

Can the authors explain how delta i_p oscillates between the values of 0 - 120 degrees?

RESPONSE: We have edited the text (that was incorrect) so that we call this angle the mutual inclination of the planets that is defined by what is now equation 2.

15) Fig 4. and 7. The fontsize of labels and ticks are very small compared to the font size of the text.

RESPONSE: We have enlarged the fontsize of labels and ticks in both Fig 4. and 7.


16) Fig. 4

The right panel shows an unstable configuration (i_p = 67.5, a_p2 = 18.3 a_b). The color code that corresponds to this simulation in the stability map in Fig. 3 is red, which means only the outer planet survives (according to page 3, line 49, left column).

However, the upper left panel in Fig. 4 for this simulation shows that the eccentricity of both planets exceeds 0.99, hence none of the planets survive.
Shouldn't the color code be white?

Can the authors confirm that the color code assignment works well for other simulations?

RESPONSE: Thank you for noticing this inconsistency. We have updated Fig. 4. The pixels in Figure 3 are correct. When we simulated the unstable case again to make figure 4, we didn’t remove the unstable inner planet and it resulted in numerical error that caused the outer planet to become unstable later on. For the same simulation on the stability map, we did remove the unstable inner planet and thus, the red pixel is correct in the map. We have updated the panel in figure 4 and address it in the caption.

17) 
Page 6, line 60, right column

The sentences starting with "For the i_p = 30 and 90 cases," ends with telling that the configurations of these two cases are stable.

For i_p = 90, the results look stable indeed.

However, for the case of i_p = 30, the oscillation of the parameters is not following a repeating trend. There is a probability that the system can get unstable if the total integration time would be longer.

To check the probability of the system being unstable, can the authors rerun this particular simulation in a longer integration time?

RESPONSE: We have run the simulation with i_p = 30 deg. five times longer and confirmed it is stable. We also update the result in the panel of Fig.7. The reason why the oscillation of the parameters is not following a repeating trend is because the e_b = 0.5. Thus, there are two orbital interactions occurring in this system i) the tilt oscillation between two planets and ii) the nodal oscillation between individual planet to the binary. We have found this unusual behaviour in a previous study (see Fig.6 in Chen et al. 2021). Moreover, we added sentences to describe it in the third paragraph of Sec. 3.4.



18) Fig. 8
The final eccentricities of some of the cases where both planets survive are very large e >> 0. However, for all the simulations the initial eccentricities are zero (circular orbits). Therefore these planets approached the limits of bounded orbits within the total integration time.

If the total integration time was longer than their selected values, these planets may be expelled from the system. However, with the selected integration time they are now considered as stable.

It should clearly be written in the manuscript that the selection of total integration time is very important, if only the survival of the planets are the basis of stability criteria.


RESPONSE: We add several sentences at the end of the first paragraph in Sec. 6 to explain that the planets on extremely eccentric orbits may become unstable later and the integration time we selected may not be able to capture the final outcome. 

19) The approach to investigate the stability in this study, depends on the survival of individual objects, and not based on any kind of stability indicator. For this reason, there is no guarantee that any surviving system actually conserves their initial condition.

As can be seen in Fig. 9, an important portion of the simulations ended with different semi-major axes compared to the initial ones, hence their orbital periods also changed.

In the stability maps (Fig. 2, 3, 5) the axes show the initial values of inclination and semi-major axes. Since the orbital periods changed, vertical axes do not represent the final stable configurations.

This can significantly alter the interpretations based on these stability maps.

For a random example, for Model X3, there is a stable region around a_p2 = 7.5 and i_p = 60 degrees. Is the final stable configuration around this region really corresponds to a_p2 = 7.5 and i_p = 60 degrees? What if the semi-major axes get 1.5 times larger for one of the planets before reaching stability?

Most of the simulations ended up in the 0.5 - 1.5 range of final a_p / initial a_p. 
If we ignore the remaining simulations and make a stability map for the final values, the range of a_p2 axis i.e. for Model X3 could be between 3 - 15 a_b instead of 6 - 10 a_b.

I think that the authors need to refer to this problem in their manuscript.

RESPONSE: We thank referee for mentioning the final distribution of the planet. Indeed, planets may not retain at their initial configuration at the end of the simulation even if two planets end up in stable orbits. We have added Fig. 10 and
several sentences at the third paragraph in Discussion and Conclusion. The figure shows that most of the case are very close to their initial positions, but in some cases, inner planets are scattered inward while outer planets are scattered outward and vice versa.

20) Page 8, line 11, right column

I suggest removing the following sentence.

"The ZKL mechanism in circumbinary planetary systems has not been thoroughly investigated before."

RESPONSE: We have removed this sentence in this paragraph.

21) Section 4.2
It may be better to rename the cases where only one planet survives as something like "one planet survivor cases" instead of "one stable planet cases", since these systems' orbital interactions have been quite chaotic.

RESPONSE: We have changed the title of Sec. 4.2 to one planet survivor cases and some texts in this subsection.

22) Page 9, line 39

Please mention what the following sentence says also in Section 2.

"In this study, we do not allow for collisions or resolve the formation of S-type planets (planets that orbit around one star of a binary) in our simulations."

RESPONSE: We have added a sentence at the third paragraph of Sec. 2 to indicate it.


23) Page 10, line 43, left column

"There are three systems KIC 07177553, KIC 7821010 and KIC 94721714 that may have a planetary-mass object orbiting around in a misaligned orbit around a binary (Borkovits et al. 2016)."

I have failed to find the binary with an ID of KIC 94721714. Can the authors check this ID?
In their work Borkovits et al. 2016 mentions KIC 9472174 in their section 6.4, instead of KIC 94721714. Maybe they made a typo in their work.
9472174
RESPONSE: We found KIC 94721714 in Borkovits et al. 2012, Borkovits et al. 2015 and Borkovits et al. 2016 but also failed to find this system on another place. We will email to the author to check whether there is a typo for KIC 9472174. In this manuscript, we replaced KIC 94721714 with KIC 9472174 at this moment.




